SpectralCanary: Embarrassingly Simple Low-Frequency Traces for T2I Dataset-Use Auditing

Auditing whether a text-to-image (T2I) model was fine-tuned on a particular image collection is difficult: a model can absorb collection-level visual characteristics without reproducing training images. Proactive dataset-use auditing plants a shared signal in a dataset before release, then later checks whether that signal appears in a suspect model's generated outputs. Existing approaches often trade off verifiability, fidelity, robustness, and deployability. We introduce $\textbf{SpectralCanary}$, which uses a smooth low-pass mask to blend a fixed canary image into every collection image while leaving captions unchanged and requiring neither auxiliary generation nor per-image optimization. A lightweight verifier detects the transferred signal in suspect-model outputs. Across eight tests on the Pokemon dataset and three realistic data transformations, spanning two architectures families, SpectralCanary achieves the highest average per-generation TPR@$1\%$ FPR ($91.1\%$) and fixed threshold model-level accuracy using 30 generations ($94.8\%$) among the evaluated methods. Across five datasets spanning artistic, medical, satellite, and fashion domains with SD3.5, SpectralCanary averages $92.4\%$ per-generation TPR@$1\%$ FPR while preserving the released images (SSIM $0.989$, LPIPS $0.022$) with a near-zero mean change FID (mean $\Delta$FID $0.05$) across datasets. Matched-energy ablations on Pokemon and ROCOv2 support our design choice, low-frequency placement transfers more reliably compared to mid/high-frequency placement. Under the evaluated adaptive attacks, the most effective removal requires aggressive modification and incurs more than $25$ $\Delta$FID points. These results identify low-frequency visual signals as effective carriers for collection-level T2I audit traces.

==> assets/coordination-figure.tex <==
\begin{tikzpicture}[x=1cm,y=1cm,font=\sffamily\small,
  nodebox/.style={minimum width=3.7cm,minimum height=1cm,align=center},
  flow/.style={-{Stealth[length=5pt]},draw=APDark,line width=0.65pt}]
  \node[nodebox] (human) at (0,0) {\textbf{Human direction}\\[-1pt]\scriptsize Objectives and constraints};
  \node[nodebox] (agents) at (5.2,0) {\textbf{Agent coordination}\\[-1pt]\scriptsize Proposals and assignments};
  \node[nodebox] (eval) at (10.4,0) {\textbf{Evaluation}\\[-1pt]\scriptsize Evidence and feedback};
  % Explicit border anchors locate the arrow-start squares in either layout.
  \draw[flow] (human.east)--(agents.west);
  \apstart{human.east}
  \draw[flow] (agents.east)--(eval.west);
  \apstart{agents.east}
  % Name the two turns to place square junctions precisely in either layout.
  \coordinate (feedback-right) at ([yshift=-0.53cm]eval.south);
  \coordinate (feedback-left) at (agents.south |- feedback-right);
  \draw[flow] (eval.south)--(feedback-right)--(feedback-left)--(agents.south);
  \apstart{eval.south}
  \apbend{feedback-right}
  \apbend{feedback-left}
  \node[fill=white,inner sep=2pt,font=\ttfamily\tiny,text=APGray] at (7.8,-1.16) {UPDATE};
\end{tikzpicture}


==> assets/diagram-style.tex <==
% Load after TikZ. Mark an explicit right-angle turn with \apbend{coordinate};
% use \apbend[APAccent]{coordinate} to match a differently colored connector.
% Square connector markers are part of both paper and cover layouts.
% Mark an arrow's starting border with \apstart{node.east} or {node.south}.
\providecommand{\apbend}[2][APDark]{%
  \path[fill=#1,draw=none]
    ([xshift=-1.5pt,yshift=-1.5pt]#2) rectangle
    ([xshift=1.5pt,yshift=1.5pt]#2);
}
\providecommand{\apstart}[2][APDark]{\apbend[#1]{#2}}


==> design2.tex <==
% !TeX program = xelatex
% COVER LAYOUT PREVIEW (legacy filename: design2.tex)
% Overleaf: select this file as Main document; use XeLaTeX as Compiler.
% Separate ruled cover page; Introduction starts on page 2.
% Edit the manuscript and its options in main.tex. This wrapper forces only
% layout=cover, inheriting main.tex's theme, logo placement and all content.
% The default wordmark is below the abstract; add logo=top in main.tex to move
% it above the title. Main.tex contains the complete commented option guide.
% For a new paper, edit starter.tex and use layout=cover on its class line;
% these wrappers preview main.tex, not starter.tex.
\def\APResearchDesignOverride{2}
\input{main.tex}

